Interaction-Transformation Evolutionary Algorithm for Symbolic Regression

The Interaction-Transformation (IT) is a new representation for Symbolic Regression that restricts the search space into simpler, but expressive, function forms. This representation has the advantage of creating a smoother search space unlike the space generated by Expression Trees, the common representation used in Genetic Programming. This paper introduces an Evolutionary Algorithm capable of evolving a population of IT expressions supported only by the mutation operator. The results show that this representation is capable of finding better approximations to real-world data sets when compared to traditional approaches and a state-of-the-art Genetic Programming algorithm.

==> pvals_old.tex <==
\begin{table}[ht]
\centering
\caption{Airfoil} 
\label{tab:pval1}
\begin{tabular}{rlllll}
  \hline
 & dCART & FEAT & GP2 & GSGP & ITEA \\ 
  \hline
FEAT & {\bf 2.5e-16} &  &  &  &  \\ 
  GP2 & {\bf 2.8e-04} & {\bf 3.6e-15} &  &  &  \\ 
  GSGP & 9.7e-01 & 9.7e-01 & 1.0e+00 &  &  \\ 
  ITEA & {\bf 2.5e-16} & {\bf 7.6e-15} & {\bf 5.1e-16} & 9.7e-01 &  \\ 
  SymTree & {\bf 4.5e-05} & {\bf 4.5e-05} & {\bf 5.0e-05} & 1.0e+00 & {\bf 7.8e-04} \\ 
   \hline
\end{tabular}
\end{table}
% latex table generated in R 3.2.3 by xtable 1.8-2 package
% Mon Mar 23 07:23:05 2020
\begin{table}[ht]
\centering
\caption{Concrete} 
\label{tab:pval2}
\begin{tabular}{rlllll}
  \hline
 & dCART & FEAT & GP2 & GSGP & ITEA \\ 
  \hline
FEAT & {\bf 2.5e-16} &  &  &  &  \\ 
  GP2 & {\bf 2.5e-16} & {\bf 2.5e-16} &  &  &  \\ 
  GSGP & 9.7e-01 & 9.7e-01 & 1.0e+00 &  &  \\ 
  ITEA & {\bf 2.5e-16} & 1.5e-01 & {\bf 2.5e-16} & 9.7e-01 &  \\ 
  SymTree & {\bf 3.5e-08} & {\bf 4.9e-04} & {\bf 3.5e-08} & 1.0e+00 & {\bf 3.7e-02} \\ 
   \hline
\end{tabular}
\end{table}
% latex table generated in R 3.2.3 by xtable 1.8-2 package
% Mon Mar 23 07:23:05 2020
\begin{table}[ht]
\centering
\caption{Energy Cooling} 
\label{tab:pval3}
\begin{tabular}{rlllll}
  \hline
 & dCART & FEAT & GP2 & GSGP & ITEA \\ 
  \hline
FEAT & {\bf 2.5e-16} &  &  &  &  \\ 
  GP2 & {\bf 2.5e-16} & {\bf 2.5e-16} &  &  &  \\ 
  GSGP & 9.7e-01 & 9.7e-01 & 1.0e+00 &  &  \\ 
  ITEA & {\bf 2.5e-16} & {\bf 4.8e-02} & {\bf 2.5e-16} & 9.7e-01 &  \\ 
  SymTree & {\bf 3.5e-08} & 1.0e+00 & {\bf 3.5e-08} & 1.0e+00 & 9.2e-02 \\ 
   \hline
\end{tabular}
\end{table}
% latex table generated in R 3.2.3 by xtable 1.8-2 package
% Mon Mar 23 07:23:05 2020
\begin{table}[ht]
\centering
\caption{Energy Heating} 
\label{tab:pval4}
\begin{tabular}{rlllll}
  \hline
 & dCART & FEAT & GP2 & GSGP & ITEA \\ 
  \hline
FEAT & {\bf 2.5e-16} &  &  &  &  \\ 
  GP2 & {\bf 5.1e-16} & {\bf 5.1e-16} &  &  &  \\ 
  GSGP & 9.7e-01 & 9.7e-01 & 1.0e+00 &  &  \\ 
  ITEA & {\bf 2.5e-16} & {\bf 7.7e-03} & {\bf 5.1e-16} & 9.7e-01 &  \\ 
  SymTree & {\bf 3.5e-08} & {\bf 7.3e-04} & {\bf 4.7e-08} & 1.0e+00 & {\bf 2.2e-02} \\ 
   \hline
\end{tabular}
\end{table}
% latex table generated in R 3.2.3 by xtable 1.8-2 package
% Mon Mar 23 07:23:05 2020
\begin{table}[ht]
\centering
\caption{Tower Data} 
\label{tab:pval5}
\begin{tabular}{rlllll}
  \hline
 & dCART & FEAT & GP2 & GSGP & ITEA \\ 
  \hline
FEAT & {\bf 2.5e-16} &  &  &  &  \\ 
  GP2 & {\bf 5.1e-16} & {\bf 5.1e-16} &  &  &  \\ 
  GSGP & 9.7e-01 & 9.7e-01 & 1.0e+00 &  &  \\ 
  ITEA & {\bf 2.5e-16} & {\bf 7.3e-05} & {\bf 5.1e-16} & 9.7e-01 &  \\ 
  SymTree & {\bf 6.5e-04} & 1.0e+00 & {\bf 7.3e-04} & 1.0e+00 & 1.0e+00 \\ 
   \hline
\end{tabular}
\end{table}
% latex table generated in R 3.2.3 by xtable 1.8-2 package
% Mon Mar 23 07:23:05 2020
\begin{table}[ht]
\centering
\caption{Wine Red} 
\label{tab:pval6}
\begin{tabular}{rlllll}
  \hline
 & dCART & FEAT & GP2 & GSGP & ITEA \\ 
  \hline
FEAT & {\bf 1.3e-16} &  &  &  &  \\ 
  GP2 & {\bf 3.8e-10} & {\bf 2.8e-06} &  &  &  \\ 
  GSGP & 9.4e-01 & 9.7e-01 & 1.0e+00 &  &  \\ 
  ITEA & {\bf 1.3e-16} & 1.0e+00 & {\bf 7.8e-06} & 9.7e-01 &  \\ 
  SymTree & {\bf 4.1e-05} & 1.0e+00 & {\bf 1.0e-03} & 1.0e+00 & 1.0e+00 \\ 
   \hline
\end{tabular}
\end{table}
% latex table generated in R 3.2.3 by xtable 1.8-2 package
% Mon Mar 23 07:23:05 2020
\begin{table}[ht]
\centering
\caption{Wine White} 
\label{tab:pval7}
\begin{tabular}{rllll}
  \hline
 & dCART & FEAT & GP2 & GSGP \\ 
  \hline
FEAT & {\bf 1.7e-16} &  &  &  \\ 
  GP2 & {\bf 8.1e-10} & {\bf 3.0e-10} &  &  \\ 
  GSGP & 1.0e+00 & 6.5e-01 & 1.0e+00 &  \\ 
  ITEA & {\bf 1.7e-16} & {\bf 2.9e-03} & {\bf 3.0e-10} & 6.5e-01 \\ 
   \hline
\end{tabular}
\end{table}
% latex table generated in R 3.2.3 by xtable 1.8-2 package
% Mon Mar 23 07:23:05 2020
\begin{table}[ht]
\centering
\caption{Yacht} 
\label{tab:pval8}
\begin{tabular}{rlllll}
  \hline
 & dCART & FEAT & GP2 & GSGP & ITEA \\ 
  \hline
FEAT & {\bf 2.5e-16} &  &  &  &  \\ 
  GP2 & {\bf 4.5e-10} & {\bf 1.5e-09} &  &  &  \\ 
  GSGP & 9.7e-01 & 9.7e-01 & 1.0e+00 &  &  \\ 
  ITEA & {\bf 2.5e-16} & 1.0e+00 & {\bf 1.8e-09} & 9.7e-01 &  \\ 
  SymTree & {\bf 4.5e-05} & {\bf 4.5e-05} & 1.0e+00 & 1.0e+00 & {\bf 6.1e-05} \\ 
   \hline
\end{tabular}
\end{table}


==> resultsTables.tex <==




%% Tabelas antigas
\iffalse
\begin{table}[t!]
\caption{Mean RMSE and Std. Dev. of the training set.}
\label{tab:resultstrain}
\centering
\begin{tabular}{l>{$}r<{$}>{$}r<{$}>{$}r<{$}>{$}r<{$}>{$}r<{$}>{$}r<{$}>{$}r<{$}>{$}r<{$}}
\toprule
%&  \multicolumn{8}{c}{\textbf{Dataset }} \\
\textbf{Algorithm} &  \text{Airfoil} &  \text{Concrete} &  \text{Cooling} &  \text{Heating} &  \text{Tower} &  \text{Red} &  \text{White} &   \text{Yacht} \\
\midrule
ITEA       & 2.36 \pm 0.05 & 5.78 \pm 0.11 & 1.51 \pm 0.04 & 0.50 \pm 0.04 & 22.11 \pm 0.45 & 0.60 \pm 0.01 & 0.71 \pm 0.00 & 0.48 \pm 0.04 \\
SymTree    &   2.05 \pm 0.06 &   5.25 \pm 0.38 &  1.57 \pm 0.03 &  0.59 \pm 0.07 &  19.83 \pm 2.05 &  0.58 \pm 0.01 &           - &  1.45 \pm 0.49 \\
FEAT       &   3.06 \pm 0.33 &   6.00 \pm 0.29 &  1.60 \pm 0.04 &  0.47 \pm 0.01 &  20.46 \pm 1.92 &  0.63 \pm 0.01 &  0.73 \pm 0.01 &  0.54 \pm 0.13 \\
dCGP      &   7.15 \pm 0.32 &  18.57 \pm 0.71 &  12.62 \pm 0.76 &  13.46 \pm 0.56 &  101.77 \pm 6.54 &  0.87 \pm 0.03 &  0.92 \pm 0.02 &  19.11 \pm 1.86 \\
GP        &   6.47 \pm 2.61 &   9.82 \pm 1.75 &   3.40 \pm 0.63 &     3.22 \pm 0.83 &   58.87 \pm 9.53 &  0.73 \pm 0.04 &  0.83 \pm 0.03 &   2.86 \pm 1.86 \\
GSGP       &  11.49 \pm 1.20 &   8.51 \pm 0.50 &  3.11 \pm 0.05 &  2.69 \pm 0.06 &  46.68 \pm 1.70 &  0.63 \pm 0.01 &  0.73 \pm 0.00 &  6.54 \pm 0.37 \\
\midrule
Forest    &  1.87 \pm 0.02 &  3.13 \pm 0.06 &  1.30 \pm 0.03 &  0.45 \pm 0.02 &  13.06 \pm 0.42 &  0.35 \pm 0.00 &  0.53 \pm 0.00 &  0.45 \pm 0.02 \\
Tree      &  2.11 \pm 0.10 &  3.12 \pm 0.18 &  1.69 \pm 0.07 &  0.38 \pm 0.09 &  13.64 \pm 0.45 &  0.58 \pm 0.03 &  0.71 \pm 0.01 &  0.66 \pm 0.31 \\
kNN       &  5.17 \pm 0.05 &  6.32 \pm 0.51 &  1.60 \pm 0.04 &  1.94 \pm 0.03 &   9.83 \pm 0.10 &  0.63 \pm 0.02 &  0.70 \pm 0.00 &  0.00 \pm 0.00 \\
\midrule
ElNet &   4.84 \pm 0.04 &  10.35 \pm 0.11 &  3.65 \pm 0.03 &  3.42 \pm 0.05 &  43.63 \pm 0.15 &  0.65 \pm 0.01 &  0.75 \pm 0.00 &  8.94 \pm 0.16 \\
Lars       &   4.80 \pm 0.04 &  10.35 \pm 0.11 &  3.18 \pm 0.02 &  2.92 \pm 0.04 &  29.58 \pm 0.75 &  0.65 \pm 0.01 &  0.75 \pm 0.00 &  8.87 \pm 0.16 \\
Lasso      &   4.80 \pm 0.04 &  10.35 \pm 0.11 &  3.18 \pm 0.02 &  2.92 \pm 0.04 &  30.07 \pm 0.73 &  0.65 \pm 0.01 &  0.75 \pm 0.00 &  8.87 \pm 0.16 \\
Ridge      &   4.85 \pm 0.04 &  10.34 \pm 0.11 &  3.21 \pm 0.03 &  2.94 \pm 0.04 &  29.59 \pm 0.74 &  0.65 \pm 0.01 &  0.75 \pm 0.00 &  8.85 \pm 0.16 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[t!]
\caption{Mean RMSE and Std. Dev. of the test set. The best result of each section is highlighted in bold with the exception of the Linear Regression, that are all very close to each other.}
\label{tab:resultstest}
\centering
\begin{tabular}{l>{$}r<{$}>{$}r<{$}>{$}r<{$}>{$}r<{$}>{$}r<{$}>{$}r<{$}>{$}r<{$}>{$}r<{$}}
\toprule
%&  \multicolumn{8}{c}{\textbf{Dataset }} \\
\textbf{Algorithm} &  \text{Airfoil} &  \text{Concrete} &  \text{Cooling} &  \text{Heating} &  \text{Tower} &  \text{Red} &  \text{White} &   \text{Yacht} \\
\midrule
ITEA &  2.50 \pm 0.15 & 6.28 \pm 0.39 & \mathbf{1.61 \pm 0.12} & 0.52 \pm 0.06 & 22.57 \pm 0.89 & 0.68 \pm 0.08 & \mathbf{0.74 \pm 0.06} & \mathbf{0.71 \pm 0.50}  \\
SymTree &   \mathbf{2.20 \pm 0.19} &   \mathbf{5.99 \pm 0.28} &  1.62 \pm 0.14 &  0.61 \pm 0.06 &   \mathbf{21.42 \pm 2.74} &  \mathbf{0.64 \pm 0.03} &  - &  1.78 \pm 0.44 \\
FEAT  &   3.18 \pm 0.31 &   6.35 \pm 0.28 &  1.63 \pm 0.12 &  \mathbf{0.49 \pm 0.05} &   25.00 \pm 9.85 &  0.65 \pm 0.03 &  0.76 \pm 0.08 &  0.83 \pm 0.22 \\
dCGP      &   7.15 \pm 0.34 &  18.56 \pm 0.69 &  12.63 \pm 0.71 &  13.46 \pm 0.60 &  101.76 \pm 6.62 &  0.85 \pm 0.02 &  0.92 \pm 0.03 &  19.13 \pm 1.84 \\
GP        &   6.63 \pm 2.79 &   9.94 \pm 1.72 &   3.46 \pm 0.69 &     3.24 \pm 0.83 &      59.14 \pm 9.56 &  0.73 \pm 0.05 &  0.83 \pm 0.03 &   3.12 \pm 2.35 \\
GSGP       &  11.62 \pm 1.32 &   9.01 \pm 0.85 &  3.17 \pm 0.15 &  2.73 \pm 0.20 &   46.76 \pm 2.47 &  0.65 \pm 0.03 &  0.74 \pm 0.01 &  6.71 \pm 1.01 \\
\midrule
%XGBoost    &   1.79 \pm 0.13 &   4.12 \pm 0.34 &  0.73 \pm 0.08 &  0.36 \pm 0.04 &   15.78 \pm 0.62 &  0.59 \pm 0.04 &  0.66 \pm 0.01 &  0.80 \pm 0.18 \\
Forest    &  \mathbf{2.43 \pm 0.07} &  \mathbf{5.33 \pm 0.31} &  \mathbf{1.80 \pm 0.12} &  \mathbf{0.59 \pm 0.10} & 17.73 \pm 1.22 &  \mathbf{0.59 \pm 0.04} &  \mathbf{0.66 \pm 0.01} &  \mathbf{1.09 \pm 0.31} \\
Tree      &  2.94 \pm 0.10 &  6.70 \pm 0.45 &  1.85 \pm 0.14 &  0.61 \pm 0.12 &  19.88 \pm 0.76 &  0.69 \pm 0.05 &  0.74 \pm 0.02 &  1.37 \pm 0.33 \\
kNN       &  6.03 \pm 0.22 &  8.91 \pm 0.97 &  1.95 \pm 0.10 &  2.34 \pm 0.37 &  \mathbf{15.06 \pm 0.92} &  0.74 \pm 0.05 &  0.81 \pm 0.02 &  7.72 \pm 1.14 \\
\midrule
ElNet &   4.87 \pm 0.15 &  10.45 \pm 0.45 &  3.70 \pm 0.13 &  3.43 \pm 0.22 &   43.74 \pm 1.25 &  0.65 \pm 0.03 &  0.75 \pm 0.01 &  9.07 \pm 0.65 \\
Lars       &   4.82 \pm 0.16 &  10.44 \pm 0.44 &  3.21 \pm 0.10 &  2.94 \pm 0.17 &   30.67 \pm 3.16 &  0.65 \pm 0.02 &  0.75 \pm 0.01 &  9.00 \pm 0.59 \\
Lasso      &   4.82 \pm 0.16 &  10.45 \pm 0.44 &  3.22 \pm 0.10 &  2.95 \pm 0.16 &   30.81 \pm 2.61 &  0.65 \pm 0.03 &  0.75 \pm 0.01 &  8.99 \pm 0.59 \\
Ridge      &   4.87 \pm 0.16 &  10.44 \pm 0.44 &  3.25 \pm 0.11 &  2.97 \pm 0.15 &   30.62 \pm 3.10 &  0.65 \pm 0.03 &  0.76 \pm 0.01 &  9.00 \pm 0.63 \\
\bottomrule
\end{tabular}
\end{table}
\fi
